Notes on kAExp(pol) problems for deterministic machines

The complexity of several logics, such as Presburger arithmetic, dependence logics and ambient logics, can only be characterised in terms of alternating Turing machines. Despite quite natural, the presence of alternation can sometimes cause neat ideas to be obfuscated inside heavy technical machinery. In these notes, we propose two problems on deterministic machines that can be used to prove lower bounds with respect to the computational class $k$AExp$_{\text{pol}}$, that is the class of all problems solvable by an alternating Turing machine running in $k$ exponential time and performing a polynomial amount of alternations, with respect to the input size. The first problem, called $k$AExp$_{\text{pol}}$-prenex TM problem, is a problem about deterministic Turing machines. The second problem, called the $k$-exp alternating multi-tiling problem, is analogous to the first one, but on tiling systems. Both problems are natural extensions of the TM alternation problem and the alternating multi-tiling problem proved AExp$_{\text{pol}}$-complete by L. Bozzelli, A. Molinari, A. Montanari and A. Peron in [GandALF, pp. 31-45, 2017]. The proofs presented in these notes follow the elegant exposition in A. Molinari's PhD thesis to extend these results from the case $k = 1$ to the case of arbitrary $k$.

==> random-stuff.tex <==

\section{Random stuff below}

\begin{itemize}
\item for every $i \in \ENat$, the logic $\QML{i}$ is a fragment of second-order modal logic, so not more expressive than graded modal logic (GML).
\item let $i,j \in \ENat$ with $i < j$. $\existsL{i}$ can be expressed in $\QML{j}$ as $\aexistsL{j}{\aprop}\bigvee_{k \leq i}\Diamond^{k}(\aprop \land \aformula)$, where $\aprop$ is an atomic proposition not occurring in~$\aformula$.
\item $\QML{1}$ is as expressive as GML. Note:
\begin{center}
  $\aexistsL{1}{\aprop_1}\dots\aexistsL{1}{\aprop_k}\bigwedge_{i \in \interval{1}{k}}\Diamond(\aformula \land \aprop_i \land \bigwedge_{j \in [i+1,k]} \lnot \aprop_j)$
\end{center}
is equivalent to $\Diamond_{\geq k} \aformula$ ($\aprop_1,\dots,\aprop_k$ not occurring in~$\aformula$). This means that, for every $i \in \ENat$, $\QML{i}$ is as expressive as GML.
\item $\exists^i \avar \aformula$ can be translated in Hybrid logic in $\downarrow \avarbis.\ \Diamond^i (\downarrow \avar.\ @_\avarbis \aformula)$, with $\avarbis$ fresh variable.
\item the satisfiability problem of $\QML{\ast}$ and the one of Sabotage Modal Logic are equireducible.

\item In $\QML{\ast}$, every formula can be put in prenex normal form:
\begin{align*}
  \Diamond \aexistsL{i}{\aprop} \aformula \ \iff \ \aexistsL{i+1}{\aprop} (\lnot \aprop \land \Diamond \aformula)\\
  \Diamond \aforallL{i}{\aprop} \aformula \ \iff \ \aexistsL{1}{\apropbis} \aforallL{i+1}\aprop \Diamond (\apropbis \land \aformula)
\end{align*}
where $\apropbis$ does not appear in $\aformula$.
\end{itemize}

\begin{lemma}
  Let $\aformula$ in $\QML{i}$ be a formula of modal depth~$m$, and with $d$ occurrences of the first-order quantification.
  There is a prenex formula $\aformulabis$ in $\QML{i+m}$ with modal depth $m$ and at most $m\cdot m$ occurrences of the first-order quantification such that $\aformula \equiv \aformulabis$.
\end{lemma}


\begin{lemma}
  Let $\aformula$ in $\fQML{\ast}$ and let $\Kripke$ be a (finite) Kripke forest. There is a deterministic time algorithm that checks whether $\Kripke \models \aformula$ 
  in time $\BigO{\card{\aformula} \cdot \card{\Kripke}^{\card{\aformula}}}$ and polynomial space.
\end{lemma}

\begin{proof}
  Simply rely on a model checking algorithm for first-order logic.
\end{proof}

\begin{lemma}
  Let $\aformula$ in $\sQML{\ast}$ and let $\Kripke$ be a (finite) Kripke forest. There is a deterministic time algorithm that checks whether $\Kripke \models \aformula$ 
  in time $\BigO{\card{\aformula} \cdot 2^{\card{\Kripke} \cdot \card{\aformula}}}$ and polynomial space.
\end{lemma}

\begin{proof}
  Simply rely on a model checking algorithm for second-order logic.
\end{proof}

Note: the model checking of second-order logic can instead be solved in $\BigO{\card{\aformula} \cdot 2^{\card{\Kripke} \cdot {\card{\aformula}}}}$.
In terms of satisfiability problem, this means that, if first-order quantification is replaced with second-order quantification, the Hierarchy should update from $\nexptime$, $2\nexptime$, $3\nexptime$ $\dots$, 
  to $\aexppol$, $2\aexppol$, $3\aexppol$ $\dots$...

==> summary.tex <==
\section{Summary of the results, and roadmap}
\label{sec:summary}

\todo[inline]{write text.}

  \begin{lemma}
    Let $\aformula$ in $\fQML{\ast}$ and let $\Kripke$ be a (finite) Kripke forest. There is a deterministic time algorithm that checks whether $\Kripke \models \aformula$ 
    in time $\BigO{\card{\aformula} \cdot \card{\Kripke}^{\card{\aformula}}}$ and polynomial space.
  \end{lemma}
  
  \begin{lemma}
    Let $\aformula$ in $\sQML{\ast}$ and let $\Kripke$ be a (finite) Kripke forest. There is a deterministic time algorithm that checks whether $\Kripke \models \aformula$ 
    in time $\BigO{\card{\aformula} \cdot 2^{\card{\Kripke} \cdot \card{\aformula}}}$ and polynomial space.
  \end{lemma}




==> thesis-macros.tex <==
%Standard Mathematical Objects
\newcommand{\pair}[2]{(#1,#2)}
\newcommand{\triple}[3]{(#1,#2,#3)}
\newcommand{\quadruple}[4]{(#1,#2,#3,#4)}
\newcommand{\tuple}[2]{(#1,\ldots,#2)}

\newcommand{\Nat}{\ensuremath{\mathbb{N}}}
\newcommand{\Rat}{\ensuremath{\mathbb{Q}}}
\newcommand{\Rea}{\ensuremath{\mathbb{R}}}
\newcommand{\Zed}{\ensuremath{\mathbb{Z}}}

\newcommand{\set}[1]{{\{ #1 \}}}
\newcommand{\powerset}[1]{2^{#1}}
\newcommand{\interval}[2]{[#1,#2]}

\renewcommand{\emptyset}{\varnothing}

\newcommand{\aset}{S}
\newcommand{\asetbis}{T}
\newcommand{\asetter}{Q}

\makeatletter
\newcommand{\dotminus}{\mathbin{\text{\@dotminus}}}

\newcommand{\@dotminus}{%
  \ooalign{\hidewidth\raise1ex\hbox{.}\hidewidth\cr$\m@th-$\cr}%
}
\makeatother

\newcommand{\proj}{\pi}

\newcommand{\arelation}{R}
\newcommand{\arelationbis}{Q}
\newcommand{\idrel}{\mathfont{id}}

\newcommand{\restrict}[2]{{#1|_{#2}}}

\newcommand{\compose}{\mathbin{\circ}}

\newcommand{\amap}{\mathfrak{f}}
\newcommand{\amapbis}{\mathfrak{g}}
\newcommand{\amapter}{\mathfrak{t}}

\newcommand{\fundots}{{:}}

\newcommand{\partarrow}{\mathbin{\rightharpoonup}}

\newcommand{\adomain}{D}
\newcommand{\acodomain}{C}

\newcommand{\txtdomain}{\mathfont{dom}}
\newcommand{\domain}[1]{\txtdomain(#1)}

\newcommand{\txtrange}{\mathfont{ran}}
\newcommand{\range}[1]{\txtrange(#1)}

\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\newcommand{\formulasize}[1]{\abs{#1}}
\newcommand{\msize}[1]{\abs{#1}_{\mathfrak{m}}}

\newcommand{\txtcard}{\mathfont{card}}
\newcommand{\card}[1]{\txtcard(#1)}

\newcommand{\fin}{\mathfont{fin}}

\newcommand{\alength}{\delta}
\newcommand{\inbound}{\beta}
\newcommand{\bound}{\alpha}

\newcommand{\isomorphism}{\simeq}

\newcommand{\egdef}{\stackrel{\text{\raisebox{-1pt}{\begin{tiny}$\mathsf{def}$\end{tiny}}}}{=}} % =def=
\newcommand{\egbydef}{\stackrel{\text{\raisebox{-1pt}{\begin{tiny}$\mathsf{by\,def}$\end{tiny}}}}{=}} % =by def=
\newcommand{\equivdef}{\stackrel{\text{\raisebox{-1pt}{\begin{tiny}$\mathsf{def}$\end{tiny}}}}{\Leftrightarrow}} % <=def=>
\newcommand{\iffbydef}{\stackrel{\text{\raisebox{-1pt}{\begin{tiny}$\mathsf{by\,def}$\end{tiny}}}}{\Leftrightarrow}} % <=def=>
\newcommand{\equivbydef}{\stackrel{\text{\raisebox{-1pt}{\begin{tiny}$\mathsf{by\,def}$\end{tiny}}}}{\equiv}} % <=by def=>
\newcommand{\eqtext}[1]{\mathbin{\raisebox{-0.4pt}{$\stackrel{\text{\raisebox{0.8pt}[0pt][0pt]{\begin{tiny}\makebox(0,0){#1}\end{tiny}}}}{=}$}}}
\newcommand{\lesstext}[1]{\mathbin{\raisebox{-0.4pt}{$\stackrel{\text{\raisebox{0.6pt}[0pt][0pt]{\begin{tiny}\makebox(0,0){#1}\end{tiny}}}}{<}$}}}

%Kripke models
\newcommand{\varprop}{{\mathsf{AP}}}
\newcommand{\avarprop}{p}
\newcommand{\avarpropbis}{q}
\newcommand{\avarpropter}{r}

\newcommand{\avaluation}{\mathcal{V}}

\newcommand{\Kripke}{\mathcal{K}}
\newcommand{\worlds}{\mathcal{W}}
\newcommand{\aworld}{\mathsf{w}}

\newcommand{\apath}{\rho}

%Decision Problems
\newcommand{\txtSAT}{\textsc{SAT}}
\newcommand{\txtVAL}{\textsc{VAL}}
\newcommand{\txtENT}{\textsc{ENT}}
\newcommand{\txtMC}{\textsc{MC}}

%Complexity classes
\newcommand{\logspace}{\textsc{LogSpace}\xspace}
\newcommand{\nlogspace}{\textsc{NLogSpace}\xspace}
\newcommand{\ptime}{\textsc{PTime}\xspace}
\newcommand{\polytime}{\ptime}
\newcommand{\lineartime}{\textsc{Lin}\xspace}
\newcommand{\np}{\textsc{NP}\xspace}
\newcommand{\conp}{\textsc{coNP}\xspace}
\newcommand{\up}{\textsc{UP}\xspace}
\newcommand{\coup}{\textsc{coUP}\xspace}
\newcommand{\pspace}{\textsc{PSpace}\xspace}
\newcommand{\atime}{\textsc{ATime}\xspace}
\newcommand{\dspace}{\textsc{DSpace}\xspace}
\newcommand{\nspace}{\textsc{NSpace}\xspace}
\newcommand{\npspace}{\textsc{NPSpace}\xspace}
\newcommand{\exptime}{\textsc{ExpTime}\xspace}
\newcommand{\nexptime}{\textsc{NExpTime}\xspace}
\newcommand{\expspace}{\textsc{ExpSpace}\xspace}
\newcommand{\twoexptime}{\textsc{2ExpTime}\xspace}
\newcommand{\twoexpspace}{\textsc{2ExpSpace}\xspace}
\newcommand{\threeexptime}{\textsc{3ExpTime}\xspace}
\newcommand{\elem}{\textsc{Elementary}\xspace}
\newcommand{\tower}{\textsc{Tower}\xspace}
\newcommand{\recurs}{\textsc{Recursive}\xspace}
\newcommand{\RE}{\textsc{RE}\xspace}
\newcommand{\aexppol}{\textsc{AExp}$_{\textsc{Pol}}$\xspace}

%Programs
\newcommand{\cif}{\textbf{if}\xspace}
\newcommand{\cpick}{\textbf{pick}\xspace}
\newcommand{\cchoose}{\textbf{choose}\xspace}
\newcommand{\cthen}{\textbf{then}\xspace}
\newcommand{\celse}{\textbf{else}\xspace}
\newcommand{\clet}{\textbf{let}\xspace}
%\newcommand{\cst}{\textbf{such that}\xspace}
\newcommand{\csatis}{\textbf{satisfying}\xspace}

%Separation Logics Fragments
\newcommand{\SL}{\mathsf{SL}}
\newcommand{\aseplog}[1]{{\SL}(#1)}
\newcommand{\qrestrict}[2]{[#1]_{#2}}
\newcommand{\prenexform}[1]{\textit{pnf-}{#1}}
\newcommand{\bsrform}[1]{\exists^*\forall^*{#1}}

  %Known fragment
  \newcommand{\FOSL}{\aseplog{\exists,\separate,\magicwand}}
  \newcommand{\FOSLNoStar}{\aseplog{\exists,\magicwand}}
  \newcommand{\FOSLNoWand}{\aseplog{\exists,\separate}}
  \newcommand{\FOSLBoundedWand}{\aseplog{\exists,\separate,\boundedwand{n}}}
  \newcommand{\QFSL}{\aseplog{\separate,\magicwand}}
  \newcommand{\QFSLNoWand}{\aseplog{\separate}}
  \newcommand{\QFSLNoWandAlloc}{\aseplog{\separate,\alloc{\avariable}}}
  \newcommand{\TwoFOSL}{\aseplog{\qrestrict{\exists}{2},\separate,\magicwand}}
  \newcommand{\OneFOSL}{\aseplog{\qrestrict{\exists}{1},\separate,\magicwand}}
  \newcommand{\OneFOSLNoWand}{\aseplog{\qrestrict{\exists}{1},\separate}}
  \newcommand{\OneFOSLNoWandAlloc}{\aseplog{\qrestrict{\exists}{1},\separate,\alloc{\avariable}}}
  \newcommand{\TwoFOSLNoWand}{\aseplog{\qrestrict{\exists}{2},\separate}}
  \newcommand{\TwoFOSLNoStar}{\aseplog{\qrestrict{\exists}{2},\magicwand}}
  \newcommand{\PrenexFOSL}{\prenexform{\FOSL}}
  \newcommand{\BSRSL}{\bsrform{\FOSL}}
  \newcommand{\OneFOSLReach}{\aseplog{\qrestrict{\exists}{1},\separate,\alloc{\avariable},\txtreach}}
  \newcommand{\OneFOSLRPlus}{\aseplog{\qrestrict{\exists}{1},\separate,\alloc{\avariable},\txtreachplus}}
  \newcommand{\OneFOSLRPlusWithWand}{\aseplog{\qrestrict{\exists}{1},\separate,\magicwand,\txtreachplus}}
  \newcommand{\SLNext}{{\aseplog{\text{\small{$\nextv{\avariable}$}},\separate,\magicwand}}}
  \newcommand{\SLReachplus}{\aseplog{\separate,\magicwand,\txtreachplus}}  \newcommand{\SLReachplusNoWand}{\aseplog{\separate,\txtreachplus}}
  \newcommand{\SLReach}{\aseplog{\separate,\magicwand,\txtreach}}
  \newcommand{\SLLs}{\aseplog{\separate,\magicwand,\txtls}}
  \newcommand{\SLLsNoWand}{\aseplog{\separate,\txtls}}
  \newcommand{\SLBoundedReach}{\aseplog{\separate,\magicwand,\txtboundedreach{2},\txtboundedreach{3}}}
  \newcommand{\SLLsBoundedWand}{\aseplog{\separate,\mbox{$\boundedwand{1}$},\txtls}}
  \newcommand{\SLFST}{{\aseplog{\qrestrict{\exists}{1},\separate,[\magicwand,\txtreachplus]^{\astrongformula}_{\aweakformula}}}}

%Other Logics

\newcommand{\BI}{\normalfont{\textsf{BI}}\xspace}
\newcommand{\BBI}{\normalfont{\textsf{BBI}}\xspace}
\newcommand{\WSO}{{\normalfont{\textsf{WSO}}}\xspace}
\newcommand{\WMSO}{{\normalfont{\textsf{WMSO}}}\xspace}
\newcommand{\WMSOF}{{\normalfont{\textsf{WMSO}}^\amap}\xspace}
\newcommand{\MSO}{{\normalfont{\textsf{MSO}}}\xspace}
\newcommand{\CTL}{{\normalfont{\textsf{CTL}}}\xspace}
\newcommand{\QCTL}{{\normalfont{\textsf{QCTL}}}\xspace}
\newcommand{\QCTLT}{{\normalfont{\textsf{QCTL}}^{t}}\xspace}
\newcommand{\QCTLTI}[2]{\QCTLT(\mathsf{#1}^{#2})}
\newcommand{\msokt}{\ensuremath{\QK^{t}}\xspace}
\newcommand{\QCTLBOOL}{\QCTLT(\mathsf{EU}^{{0}})}
\newcommand{\QCTLEF}{\QCTLT(\mathsf{EF}^{{1}})}
\newcommand{\ALT}{{\normalfont{\textsf{ALT}}}\xspace}
\newcommand{\PITL}{{\normalfont{\textsf{PITL}}}\xspace}
\newcommand{\ML}{{\normalfont{\mathsf{ML}}}\xspace}
\newcommand{\AL}{{\normalfont{\mathsf{AL}}}\xspace}
\newcommand{\SAL}{{\normalfont{\mathsf{SAL}}}\xspace}
\newcommand{\GML}{{\normalfont{\textsf{GML}}}\xspace}
\newcommand{\MSL}{{\normalfont{\textsf{MSL}}}\xspace}
\newcommand{\MLH}{{\normalfont{\textsf{MLH}}}\xspace}
\newcommand{\MSLMLH}{\prescript{\raisebox{-5pt}{\normalfont{\scriptsize{\textsf{MSL}}}}}{}{\!/}_{\normalfont{\textsf{MLH}}}\xspace}
\newcommand{\MSLDMU}{\ensuremath{\MSL(\separate,\Diamond^{-1})}}

\newcommand{\SHSL}{{\normalfont{\textsf{SH}}}\xspace}
\newcommand{\SHSLLs}{{\normalfont{\textsf{SH}}(\txtls)}\xspace}


\newcommand{\tup}[1]{\langle #1 \rangle}
\newcommand{\HMDiamond}[1]{\tup{{#1}}}
\newcommand{\HMBox}[1]{[{#1}]}

%General Logical Lingua
\newcommand{\alogic}{\mathcal{L}}
\newcommand{\grammardef}{\coloneqq}

\newcommand{\true}{\top}
\newcommand{\false}{\perp}

\newcommand{\aformula}{\varphi}
\newcommand{\aformulabis}{\psi}
\newcommand{\aformulater}{\chi}
\newcommand{\aformulafour}{\gamma}

\newcommand{\positions}[1]{\ensuremath{\texttt{Pos}(#1)}}
\newcommand{\aposition}{\rho}

\renewcommand{\implies}{\Rightarrow}
\renewcommand{\iff}{\Leftrightarrow}

\newcommand{\freevars}[1]{\mathsf{fv}(#1)}
\newcommand{\boundvars}[1]{\mathsf{bv}(#1)}

\newcommand{\aliteral}{L}
\newcommand{\LIT}{\mathsf{LIT}}
\newcommand{\fstliterals}[2]{\LIT_{#2}(#1)}
\newcommand{\literals}[1]{\LIT(#1)}
\newcommand{\inside}{\subseteq_{\LIT}}
\newcommand{\orliterals}[2]{\{#1\mathbin{|}#2\}}
\newcommand{\threeorliterals}[3]{\{#1\mathbin{|}#2\mathbin{|}#3\}}
\newcommand{\threeandliterals}[3]{\{#1\mathbin{;}#2\mathbin{;}#3\}}
\newcommand{\andliterals}[2]{\{#1\mathbin{;}#2\}}

\makeatletter
\newcommand\bmat{{\ifnum\z@=`}\fi\@bmat}
\def\@bmat[#1]{%
  {{\arraycolsep=0pt\def\arraystretch{0.95}\begin{array}{r}#1\end{array}}}\ifnum\z@=`{\fi}%
}
\makeatother

\newcommand{\aformulasubset}[1]{{\scalebox{0.8}{$\left\{ #1 \right\}$}}}
\newcommand{\formulasubset}[2]{{\scalebox{0.8}{$\left\{ #1\, \middle|\, #2 \right\}$}}}

\newcommand{\scaledformulasubset}[4]{{\scalebox{#3}{$\left\{ #1\, \middle|\, {\scalebox{#4}{$#2$}} \right\}$}}}

\newcommand{\anyform}[2][]{\bm{|}#2{\bm{?}}_{\ifthenelse {\equal {#1} {}}{}{(#1)}}}


%Proof System 

\newcommand{\placeholder}{\square}
\newcommand{\aformulaschema}{\Phi}
\newcommand{\aformulaschemabis}{\Psi}
\newcommand{\asubstitution}{\sigma}

\newcommand{\aproofsystem}{\mathcal{H}}
\newcommand{\pfentails}[2]{\vdash_{#1}#2}

\newcommand{\prove}{\vdash}

%Substitutions
\newcommand{\completesubstitute}[2]{{[#2{\gets}#1]}}
\newcommand{\completesubstitutemult}[3]{{[#2{\gets}#1\mid#3]}}
\newcommand{\partialsubstitute}[2]{{\{#2{\gets}#1\}}}

%Separation Logic Lingua
\newcommand{\VAR}{\mathfont{VAR}}
\newcommand{\FOVAR}{\mathfont{FO}_{\VAR}}
\newcommand{\LOC}{\mathfont{LOC}}
\newcommand{\GLOC}{\mathfont{G}}

\newcommand{\Stores}{\mathbb{S}}
\newcommand{\Heaps}{\mathbb{H}}
\newcommand{\MemoryStates}{\mathbb{MS}}

\newcommand{\astore}{s}
\newcommand{\aheap}{h}

\newcommand{\disjoint}{\bot}
\newcommand{\heapsum}{+}
\newcommand{\subheap}{\subseteq}
\newcommand{\strictsubheap}{\subsetneq}

\newcommand{\nilvalue}{\mathtt{nil}}
\newcommand{\emp}{\mathtt{emp}}
\newcommand{\txtpto}{\mapsto}
\newcommand{\pto}[2]{{#1\,{\txtpto}\,#2}}
\newcommand{\txtIpto}{\hookrightarrow}
\newcommand{\Ipto}[2]{{#1\,{\txtIpto}\,#2}}
\newcommand{\txtboundedreach}[1]{\txtIpto^{#1}}
\newcommand{\boundedreach}[3]{{#1\,{\txtboundedreach{#3}}\,#2}}
\newcommand{\Iimplies}{\to}
\newcommand{\separate}{\mathbin{\ast}}
\newcommand{\magicwand}{\mathbin{-\mkern-6mu*}}
\newcommand{\septraction}{\mathbin{{-\mkern-8mu{\raisebox{0.6pt}{$\scriptstyle{\circledast}$}}}}}
\newcommand{\boundedwand}[1]{\mathbin{{-\mkern-4mu\raisebox{1pt}{$\scriptstyle{\left[#1\right]}$}}}}
\newcommand{\boundedseptraction}[1]{\mathbin{{-\mkern-4mu\raisebox{1pt}{$\scriptstyle{\langle#1\rangle}$}}}}

\newcommand{\Bigseparate}{\DOTSB\bigop{\resizebox{13pt}{14pt}{$\separate$}}}

\newcommand{\avariable}{\mathtt{x}}
\newcommand{\avariablebis}{\mathtt{y}}
\newcommand{\avariableter}{\mathtt{z}}
\newcommand{\avariablefour}{\mathtt{v}}
\newcommand{\avariablefive}{\mathtt{w}}
\newcommand{\avariablesix}{\mathtt{u}}

\newcommand{\uniquevar}{\mathtt{u}}

\newcommand{\asetofvars}{\mathtt{X}}
\newcommand{\asetofvarsbis}{\mathtt{Y}}
\newcommand{\asetofvarster}{\mathtt{Z}}
\newcommand{\asetofvarsfour}{\mathtt{V}}

\newcommand{\asetofterms}{\mathtt{T}}

\newcommand{\alocation}{\ell}

\newcommand{\asetoflocs}{\mathtt{L}}

\newcommand{\defined}[1]{(#1){\downarrow}}

% Auxiliary SL formulae
\newcommand{\alloc}[1]{\Ipto{#1}{\_\,}}
\newcommand{\allocback}[1]{\Ipto{\,\_}{#1}}

\newcommand{\txtsize}{\mathtt{size}}
\newcommand{\sizegeq}[1]{{\mathtt{size}\,{\geq}\,#1}}
\newcommand{\sizeeq}[1]{{\mathtt{size}\,{=}\,#1}}
\newcommand{\maxsize}[1]{\max_{\txtsize}(#1)}

\newcommand{\txtpred}{\mathtt{\#pto}}
\newcommand{\predgeq}[2]{{\mathtt{\#pto}(#1)\,{\geq}\,#2}}
\newcommand{\predeq}[2]{{\mathtt{\#pto}(#1)\,{=}\,#2}}

\newcommand{\txtls}{\mathtt{ls}}
\newcommand{\ls}[2]{\txtls(#1,#2)}

\newcommand{\txtreach}{\txtIpto^{\!*}}
\newcommand{\reach}[2]{{#1\,{\txtreach}\,#2}}

\newcommand{\txtreachplus}{\txtIpto^{\!+\!\!}}
\newcommand{\reachplus}[2]{{#1\,{\txtreachplus}\,#2}}

\newcommand{\txtreachn}[1]{\txtIpto^{\!#1}}
\newcommand{\reachn}[3]{{#1\,\txtreachn{#3}\,#2}}

\newcommand{\txtstrict}{\mathtt{strict}}
\newcommand{\strict}[1]{\txtstrict(#1)}

\newcommand{\subsize}[2]{\left[#1\right]_{#2}}

% Second-order logic
\newcommand{\amodel}{\mathcal{M}}
\newcommand{\amodeldomain}{\mathcal{D}}
\newcommand{\aassign}{r}
\newcommand{\arity}[1]{\mathfont{ar}(#1)}

  % Auxiliary predicates
    \newcommand{\functsymbol}[1]{\mathfont{fun}(#1)}
    \newcommand{\infdom}{\mathfont{Dom}[\omega]}


%Translations
\newcommand{\atranslation}{{\mbox{\larger{$\tau$}}}\!}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Undecidability chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\encodedby}[2]{\rhd^{#1}_{#2}}
\newcommand{\nextv}[1]{\mathtt{n}(#1)}
\newcommand{\marked}[1]{\overbracket[1pt][0pt]{#1}}
\newcommand{\Safe}{\mathtt{Store}}

\newcommand{\asetofmarkedvars}{\mathbb{Y}}

\newcommand{\txtalloc}{\mathtt{alloc}}
\newcommand{\allocbackaux}[2]{\txtalloc^{-1}_{#2}(#1)}
\newcommand{\txtnexteq}{\mathtt{next}}
\newcommand{\nexteq}[2]{\txtnexteq(#1 = #2)}
\newcommand{\nextpto}[3]{\txtnexteq_{#3}(\Ipto{#1}{#2})}

\newcommand{\txtselfloop}{\mathtt{self}}
\newcommand{\selfloopeq}[3]{\txtselfloop_{#2}(#1)\,{=}\,#3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  ALT chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\intree}{\mathtt{Hit}}
\newcommand{\ingarbage}{\mathtt{Miss}}

\newcommand{\auniverse}{\mathcal{N}}

\newcommand{\altmodel}[3]{\triple{#1}{#3}{#2}}

\newcommand{\atree}{\mathcal{F}}
\newcommand{\ambtree}{\mathsf{T}}

\newcommand{\treesatone}[2]{{#1}\!\left[#2\right]}
\newcommand{\treesattwo}[3]{{#1}\!\left[#3\right]_{#2}}
\newcommand{\atreesat}[1]{\treesatone{\atree}{#1}}

\newcommand{\aagarbageone}[1]{\treesatone{#1}{\ingarbage}}
\newcommand{\aagarbage}{\aagarbageone{\atree}}
\newcommand{\agarbage}[2]{\treesattwo{#1}{#2}{\ingarbage}}

\newcommand{\treeroot}{\mathsf{t}}
\newcommand{\anode}{\mathsf{n}}

\newcommand{\anodeset}{\mathsf{N}}
\newcommand{\amainpath}{\mathsf{M}}
\newcommand{\wordsets}{\mathbb{M}}
\newcommand{\charsets}{\mathbb{C}}

\newcommand{\aaefapprox}[1]{\sim_{#1}\!}
\newcommand{\efapprox}[3]{\aaefapprox{\triple{#1}{#2}{#3}}}
\newcommand{\aefapprox}{\efapprox{\modalrank}{\sabotagerank}{\sabotagestarrank}}

\DeclareMathOperator{\Diamonduniv}{\langle{\normalfont{U}}\rangle}
\DeclareMathOperator{\Boxuniv}{[\text{U}]}

\DeclareMathOperator{\SabDiamond}{\blacklozenge}
\DeclareMathOperator{\SabDiamondSL}{\SabDiamond_{\!\raisebox{0pt}[0pt][0pt]{\! \texttt{\tiny{SL}}}}^{\!\raisebox{-1.5pt}[0pt][0pt]{\scalebox{1.05}[1.05]{\hphantom{$*$}}}}\!}
\DeclareMathOperator{\SabDiamondML}{\SabDiamond_{\!\raisebox{0pt}[0pt][0pt]{\! \texttt{\tiny{ML}}}}^{\!\raisebox{-1.5pt}[0pt][0pt]{\scalebox{1.05}[1.05]{\hphantom{$*$}}}}\!}

\DeclareRobustCommand{\SabDiamondTitle}{\texorpdfstring{\SabDiamond}{BlackDiamond}}

\DeclareMathOperator{\SabBox}{\blacksquare}

\DeclareMathOperator{\SabDiamondStar}{\SabDiamond_{\!\raisebox{0pt}[0pt][0pt]{\texttt{\vphantom{\tiny{SL}}}}}^{\!\raisebox{-3.5pt}[0pt][0pt]{\scalebox{1.05}[1.05]{$*$}}}}
\DeclareMathOperator{\SabDiamondStarSL}{\SabDiamond_{\!\raisebox{0pt}[0pt][0pt]{ \texttt{\tiny{SL}}}}^{\!\raisebox{-3.5pt}[0pt][0pt]{\scalebox{1.05}[1.05]{$*$}}}}
\DeclareMathOperator{\SabDiamondStarML}{\SabDiamond_{\!\raisebox{0pt}[0pt][0pt]{ \texttt{\tiny{ML}}}}^{\!\raisebox{-3.5pt}[0pt][0pt]{\scalebox{1.05}[1.05]{$*$}}}}

\DeclareMathOperator{\SabBoxStar}{\SabBox^{\scalebox{1.05}[1.05]{$*$}}}


\newcommand{\guarantee}{\vartriangleright}
\newcommand{\guartraction}{\blacktriangleright}

\newcommand{\rankorder}{<_{\textit{rk}}}

  % Auxiliary formulae
  \newcommand{\altalloc}{\mathtt{inDom}}
  \newcommand{\treesize}{\txtsize}
  \newcommand{\monosize}[1]{\txtsize(#1)}
  \newcommand{\garbagesize}{\monosize{\ingarbage}}
  \newcommand{\garbagesizegeq}[1]{\garbagesize\,{\geq}\,#1}
  \newcommand{\monosizegeq}[2]{\monosize{#1}\,{\geq}\,#2}


  \newcommand{\atargetpred}{\mathtt{tchild}}
  \newcommand{\targetpred}{\monosize{\atargetpred}}
  \newcommand{\targetpredgeq}[1]{\monosize{\atargetpred}\,{\geq}\,#1}
  \newcommand{\targetpredeq}[1]{\monosize{\atargetpred}\,{=}\,#1}

  \newcommand{\altpred}{\mathtt{\#child}}
  \newcommand{\actchar}{\mathtt{1st}}
  \newcommand{\isword}{\mathtt{word}}
  \newcommand{\anc}{\mathtt{\#desc}}
  \newcommand{\ancgeq}[1]{\anc\,{\geq}\,#1}
  \newcommand{\anceq}[1]{\anc\,{=}\,#1}
  \newcommand{\altpredgeq}[1]{\altpred\,{\geq}\,#1}
  \newcommand{\altpredeq}[1]{\altpred\,{=}\,#1}


  % Marked stuff
  \newcommand{\ismarked}{\mathtt{mark}}
  \newcommand{\issymbol}{\mathtt{symb}}
  \newcommand{\nmarks}{\mathtt{marks}}
  \newcommand{\beforemarks}{\mathtt{\#markAnc}}
  \newcommand{\pitltranslation}{\mathsf{\nabla}\!}
  \newcommand{\alttranslation}{\mathsf{\tau}}

%GAMES

\newcommand{\modalrank}{\mathsf{m}}
\newcommand{\sabotagerank}{\mathsf{s}}
\newcommand{\sabotagestarrank}{\mathsf{k}}

\newcommand{\aformularank}{\triple{\modalrank}{\sabotagerank}{\sabotagestarrank}}

\newcommand{\arank}{\mathsf{rk}}
%\newcommand{\formularank}[1]{\mathsf{rk}(#1)}
\newcommand{\aformulaerankset}[1]{{{\ALT}_{#1}}}
\newcommand{\acharactformula}[2]{\mathsf{\Gamma}_{\!#2}{#1}}

%WORDS

\newcommand{\aalphabet}{\mathsf{\Sigma}}     % an alphabet, A is already used for atoms
\newcommand{\aword}{\mathfrak{w}}

\newcommand\achar{\mathtt{a}}
\newcommand\acharbis{\mathtt{b}}

%PITL
\newcommand\pt{\mathtt{1}}
\DeclareMathOperator{\chop}{\raisebox{-2pt}{\rule{1.2pt}{2.1ex}}}

%MARKED PITL
\newcommand{\amarkedalphabet}{\aalphabet_{\bullet}}
\newcommand\markedmodels{\models_{\bullet}}
\newcommand{\markedsplit}[1]{\Delta(#1)}

%QCTL

\newcommand{\EX}{\mathsf{EX}\,}
\newcommand{\EF}{\mathsf{EF}\,}
\newcommand{\AG}{\mathsf{AG}\,}
\newcommand{\AF}{\mathsf{AF}\,}
\newcommand{\EG}{\mathsf{EG}\,}

\newcommand{\txtEU}{\mathsf{EU}}
\newcommand{\EU}[2]{ \mathsf{E}(#1\,\mathsf{U}\,#2)}
\newcommand{\AU}[2]{ \mathsf{A}(#1\,\mathsf{U}\,#2)}
\newcommand{\EM}[2]{ \mathsf{E}(#1\,\mathsf{M}\,#2)}

\newcommand{\Paths}[2]{\Pi_{#2}(#1)}

\newcommand{\kripkeroot}{\mathsf{r}}

\newcommand{\avartree}{\texttt{\textit{D}}}
\newcommand{\avartreebis}{\texttt{\textit{E}}}
\newcommand{\avarend}{\texttt{\textit{end}}}
\newcommand{\avarnode}{\texttt{\textit{n}}}
\newcommand{\avartreeroot}{\texttt{\textit{t}}}

\newcommand{\unique}[1]{\mathtt{uniq}(#1)}
\newcommand{\monotone}[1]{\mathtt{monotone}(#1)}

\newcommand{\aterm}{\mathtt{t}}
\newcommand{\atermbis}{\textit{\texttt{u}}}

\DeclareMathOperator{\QCTLenc}{\mathtt{enc}}

%MSL

\newcommand{\spy}{\mathtt{spy}}
\newcommand{\isspy}{\mathtt{is\_a\_spy}}
\newcommand{\selfloop}{\mathtt{selfloop}}
\newcommand{\hascycles}{\mathtt{hascycles}}
\newcommand{\hasoneselfloop}{\exists\mathtt{1selfloop}}


\DeclareMathOperator{\Diamonddiff}{\langle{\neq}\rangle}
\DeclareMathOperator{\Boxdiff}{[\neq]}

\newcommand{\nom}[1]{\mathtt{nom}(#1)}
\newcommand{\fullatnom}[1]{\mathtt{@}_{#1}\,}

\newcommand{\locnom}[2]{\mathtt{nom}_{#2}(#1)}
\newcommand{\atlocnom}[2]{\mathtt{@}_{#1}^{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  FSTTCS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Strong}{\mathcal{S}}
\newcommand{\Weak}{\mathcal{W}}

\newcommand{\astrongformula}{{\scriptstyle{\Strong}}}
\newcommand{\aweakformula}{{\scriptstyle{\Weak}}}

\newcommand{\apolynomial}{\mathcal{Q}}

\newcommand{\coreformulae}[2]{\texttt{Core}(#1,#2)}
\newcommand{\coreformulaebot}[2]{\texttt{Core}_{\false}(#1,#2)}
\newcommand{\conjcomb}[1]{\texttt{Conj}(#1)}
\newcommand{\boolcomb}[1]{\texttt{Bool}(#1)}

\newcommand{\acoretype}{\texttt{CoreTypes}}
\newcommand{\coretype}[2]{\acoretype(#1,#2)}
\newcommand{\coretypebis}[2]{\acoretype'(#1,#2)}

\newcommand{\remgeq}[2]{\mathtt{rem}_{#1}\geq{#2}}

\newcommand{\hop}[2]{\leftrightarrow_{#1,#2}}

\newcommand{\alocationset}{\mathtt{L}}

\newcommand{\coreeq}{\approx}

\newcommand\BigO{\mathcal{O}}
\newcommand\PolyMW{\mathfrak{P}}
\newcommand\PolyUP{\mathfrak{Q}}
\newcommand\varcount[1]{\#\freevars{#1}}

\newcommand{\maxval}[2]{\texttt{maxval}_{#2}(#1)}

%Weak fragment
\newcommand{\TermsO}[1]{\mathtt{T}[\aweakformula]^{#1}}
\newcommand{\NextO}[1]{\mathtt{NV}[\aweakformula]^{#1}}
\newcommand{\LabsO}[2]{\mathtt{Lab}[\aweakformula]_{#1}^{#2}}

\newcommand{\SkeletonO}{\mathtt{Sk}[\aweakformula]}
\newcommand{\predO}{\mathtt{pred}^\aweakformula}
\newcommand{\loopsO}{\mathtt{self}^\aweakformula}
\newcommand{\sizeO}{\mathtt{rem}^\aweakformula}

\newcommand{\ObservedO}{\mathtt{Obs}[\aweakformula]}
\newcommand{\inpredO}{\in\predO}
\newcommand{\inloopsO}{\in\loopsO}
\newcommand{\insizeO}{\in\sizeO}

\newcommand{\TestO}{\texttt{Core}[\aweakformula]}
\newcommand{\weakeq}{\coreeq^{\aweakformula}}

\newcommand{\PREDO}{\mathtt{Pred}[\aweakformula]}
\newcommand{\SIZEO}{\mathtt{Rem}[\aweakformula]}
\newcommand{\LOOPO}{\mathtt{Self}[\aweakformula]}

\newcommand{\sem}[2]{\ensuremath{[\![#1]\!]}^{\asetofvars}_{#2}}
\newcommand{\easysem}[1]{\ensuremath{[\![#1]\!]}}
\newcommand{\weakhop}[2]{\leftrightarrow_{#1,#2}^{\aweakformula}}

\newcommand{\DIFFO}[2]{[(#1)\#_{\asetofvars}(#2)]}

%Strong fragment
\newcommand{\TermsP}[1]{\mathtt{T}[\astrongformula]^{\asetofvars}}
\newcommand{\MeetP}[1]{\mathtt{MV}[\astrongformula]^{\asetofvars}}
\newcommand{\EndP}[1]{\mathtt{EV}[\astrongformula]^{\asetofvars}}
\newcommand{\strongeq}{\coreeq^{\astrongformula}}

\newcommand{\ameetset}{\mathtt{M}}
\newcommand{\aendset}{\mathtt{E}}

\newcommand{\LabsP}[1]{\mathtt{Lab}[\astrongformula]_{#1}^{\asetofvars}}

\newcommand{\meetv}[2]{\mathtt{m}({#1,#2})}
\newcommand{\tend}[1]{\mathtt{e}({#1})}

\newcommand{\PREDP}[2]{\mathtt{Pred}[\astrongformula]^{\asetofvars}_{#1}(#2)}
\newcommand{\PATHP}[2]{\mathtt{Path}[\astrongformula]^{\asetofvars}_{#1}(#2)}
\newcommand{\apprime}{\mathtt{Path}'}
\newcommand{\LOOPP}[2]{\mathtt{Cycl}[\astrongformula]^{\asetofvars}_{#1}\!\!\left(#2\right)}
\newcommand\compactdots{\hbox to 0.8em{.\hss.\hss.}}
\newcommand{\ULOOPP}[2]{{\raisebox{1.5pt}{$\Uparrow$}}\mathtt{Cycl}[\astrongformula]^{\asetofvars,#2}_{#1}}
\newcommand{\SIZEP}[2]{\mathtt{Rem}[\astrongformula]^{\asetofvars,#2}_{#1}}
\newcommand{\muPATHP}[2]{\mathtt{sby}^{\asetofvars}_{#1}(#2)}

\newcommand{\TestP}[1]{\texttt{Core}[\astrongformula](#1)}

\newcommand{\SkeletonP}[1]{\mathtt{Sk}[\astrongformula](#1)}

\newcommand{\ObservedP}[1]{\mathtt{Obs}[\astrongformula](#1)}

\newcommand{\sees}[1]{\mathtt{sees}_{\asetofvars}(#1)}
\newcommand{\downsquigarrow}{{\mathbin{\rotatebox[origin=c]{270}{$\rightsquigarrow$}}}}
\newcommand{\loopsP}[1]{\mathtt{loop}^{\astrongformula}_{\asetofvars}(#1)}
\newcommand{\unbloop}[1]{{\raisebox{1.5pt}{$\Uparrow$}}\mathtt{loop}^{\astrongformula}_{\asetofvars,#1}}
\newcommand{\predP}[1]{\mathtt{pred}^{\astrongformula}_{\asetofvars}(#1)}
\newcommand{\sizeP}[1]{\mathtt{rem}^{\astrongformula}_{\asetofvars,#1}}

\newcommand{\insees}[1]{\in\sees{#1}}
\newcommand{\inloopsP}[1]{\in\loopsP{#1}}
\newcommand{\inpredP}[1]{\in\predP{#1}}
\newcommand{\insizeP}[1]{\in\sizeP{#1}}
\newcommand{\inunbloop}[1]{\in\unbloop{#1}}

\newcommand{\stronghop}[2]{\leftrightarrow_{#1,#2}^{\astrongformula}}

\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcN}{\mathcal{N}}

\newcommand\loopUB[1]{\mathcal{L}(#1)}
\newcommand\sizeUB[1]{\mathcal{R}(#1)}
\newcommand\predUB[1]{\mathcal{P}(#1)}
\newcommand\RbtwnUB[1]{\mathcal{S}_{\text{right}}(#1)}
\newcommand\LbtwnUB[1]{\mathcal{S}_{\text{left}}(#1)}
\newcommand\seesUB[1]{\mathcal{S}(#1)}

\newcommand{\satDP}[1]{\texttt{sat(}#1\texttt{)}}
\newcommand{\mcDP}[1]{\texttt{mc(}#1\texttt{)}}
\newcommand{\atomicDP}[1]{\texttt{atomic\_mc(}#1\texttt{)}}
\newcommand{\mcSPACE}[1]{\texttt{SPACE}\left[#1\right]}

\newcommand{\algsucceed}{\texttt{succeed}\xspace}
\newcommand{\algfail}{\texttt{fail}\xspace}

\newcommand{\alldiff}[1]{\mathtt{alldiff}(#1)}
\newcommand{\alldiffGML}[1]{\mathtt{alldiff}_{\GML}(#1)}
\newcommand{\alleq}[1]{\mathtt{alleq}(#1)}
\newcommand{\lostterm}[1]{\mathtt{unlab}(#1)}
\newcommand{\seenisvar}[1]{\mathtt{var.sby}(#1)}

\newcommand{\strongalloc}[1]{\mathtt{alloc}_{\astrongformula}(#1)}
\newcommand{\strongIpto}[2]{{#1\,{\txtIpto_{\astrongformula}}\,#2}}
\newcommand{\strongreachplus}[2]{{#1\,{\txtreachplus_{\astrongformula}}\,#2}}
\newcommand{\strongreach}[2]{{#1\,{\txtreach_{\astrongformula}}\,#2}}

\newcommand{\seespath}[1]{\mathtt{seeslen}_{\asetofvars}(#1)}

\newcommand{\isvar}[1]{\mathtt{var}_{\asetofvars}(#1)}
\newcommand{\isnext}[1]{\mathtt{next}_{\asetofvars}(#1)}
\newcommand{\termself}[1]{\mathtt{self}_{\asetofvars}(#1)}

\newcommand{\DIFFP}[2]{[(#1)\#_{\asetofvars,\bound}(#2)]}

%\newcommand{\sharpvar}[1]{\mathsf{\#v}(#1)}

\newcommand{\flatted}[1]{[#1]^{\flat}}

\newcommand{\aREset}{\texttt{Rem}}
\newcommand{\aLset}{\texttt{Lft}}
\newcommand{\aRset}{\texttt{Rgt}}

\newcommand{\aRRRset}{\texttt{RR}}

\newcommand{\deltaL}{\alength_{\textit{lft}}}
\newcommand{\deltaR}{\alength_{\textit{rgt}}}

\newcommand{\aheapL}{\aheap_{\textit{pre}}}
\newcommand{\aheapC}{\aheap_{\textit{ct}}}
\newcommand{\aheapR}{\aheap_{\textit{sfx}}}

\newcommand{\aremset}{R}
\newcommand{\apathset}{P}
\newcommand{\aseesset}{S}
\newcommand{\aloopset}{C}
\newcommand{\apredset}{P}
\newcommand{\aunbset}{U}

\newcommand{\apropset}{P}
\newcommand{\apropsetbis}{Q}
\newcommand{\apropsetter}{T}
\newcommand{\apropsetN}{\mathsf{N}}

\newcommand{\aremheap}{\textsc{r}}
\newcommand{\aseesheap}{\textsc{s}}
\newcommand{\aloopheap}{\textsc{c}}
\newcommand{\apredheap}{\textsc{p}}
\newcommand{\aunbheap}{\textsc{u}}

\newcommand{\aremloc}{\alocation_{\texttt{r}}}


\newcommand{\apathpred}{\normalfont{l}_\textit{pre}}

\newcommand{\apathend}[1]{\normalfont{e}_{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Axiomatisation Chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{tcolorbox}

\tcbset{
halign title = left,
left=0pt,
right=0pt,
top=0pt,
bottom=0pt,
colback=black!3,
colframe=black!3,
coltitle=black,
fonttitle=\small,
boxrule=0pt,
width=\dimexpr\textwidth\relax,
enlarge left by=0mm,
boxsep=1pt,
arc=0pt,outer arc=0pt,
before upper={\hrule\smallskip},
after upper={\smallskip\hrule}
}

\newtcolorbox[auto counter]{axiombox}[2][]{title=(System~\thetcbcounter)\ #2,#1}


\newcommand{\corepedix}{\mathsf{C}}
\newcommand{\coresys}{\aproofsystem_{\corepedix}}
\newcommand{\starsys}{\coresys(\separate)}
\newcommand{\magicwandsys}{\coresys(\separate,\magicwand)}

\newcommand{\assuming}[1]{\ \blacktriangleleft\!\!\!\left[#1\right]}

\newcommand{\inference}[3][]{\text{#1}\frac{\displaystyle #2}{\displaystyle #3}}

\newcommand{\aelement}{\mathtt{e}}

\newcommand{\boxbin}[3]{{\langle\mbox{$#1$}\rangle}(#2,#3)}
\newcommand{\boxstar}[2]{\boxbin{\separate}{#1}{#2}}
\newcommand{\boxseptra}[2]{\boxbin{\septraction}{#1}{#2}}

\newcommand{\ALLOC}{\textsf{\small{ALLOC}}}
\newcommand{\UNALLOC}{\textsf{\small{U}}}
\newcommand{\GARB}{\textsf{\small{GARB}}}

\newcommand{\ATOM}[1]{\textsf{\small{ATOM}}(#1)}
\newcommand{\SMALLATOM}[2]{\textsf{\small{A}}_{#2}(#1)}
\newcommand{\ALMOST}[1]{\textsf{\small{ALMOST}}(#1)}

\newcommand{\aforUNALLOC}{\aformula_{\lnot\texttt{alloc}}}
\newcommand{\aforEQ}{\aformula_{\texttt{(in)eq}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Ambient Logic Chapter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\ATM}{\ensuremath{\normalfont{\mathsf{ATM}}}\xspace}

\newcommand{\MA}{\ensuremath{\normalfont{\mathsf{MA}}}\xspace}
\newcommand{\MLChop}{{\ensuremath{\ML(\,\chopop\,)}}\xspace}
\newcommand{\fragmentF}{\mathcal{F}}
\newcommand{\MLCG}{{\ensuremath{\ML(\,\chopop\,,\guarantee)}}\xspace}
\newcommand{\chopop}{\mathbin{\raisebox{-2pt}{\rule{1.2pt}{2.1ex}}}}
\newcommand{\txtSAL}{\mathsf{SAL}}
\newcommand{\SALC}{{\ensuremath{\txtSAL(\,\chopop\,)}}\xspace}

\newcommand{\ncoretype}[3]{\acoretype^{#1}(#2,#3)}

\newcommand{\GMLsys}{\aproofsystem_{\mathsf{GML}}}
\newcommand{\compsys}{\GMLsys(\text{\footnotesize$\,\chopop\,$})}
\newcommand{\guaranteesys}{\GMLsys(\text{\footnotesize$\,\chopop\,$},\guarantee)}

\newcommand{\md}[1]{{\mathsf{md}}(#1)}
\newcommand{\bd}[1]{\mathsf{bd}(#1)}
\newcommand{\topbd}[1]{{\mathsf{top}}_{\mathsf{bd}}(#1)}
\newcommand{\newbd}[2]{{\mathsf{bd}}(#1,#2)}
\newcommand{\gr}[1]{{\mathsf{gr}}(#1)}
\newcommand{\rank}[1]{{\mathsf{rank}}(#1)}
\newcommand{\veeweight}[1]{{\mathsf{w}}_{\plvee}(#1)}
\newcommand{\maxbd}[1]{{\mathsf{max}}_{\mathsf{bd}}(#1)}
\newcommand{\submax}[1]{{\mathsf{submax}}_{\mathsf{GM}}(#1)}
\newcommand{\cd}[1]{{\mathsf{cd}}(#1)} %% composition degree / depth
\newcommand{\dweight}[1]{{\mathsf{w}}_{\Diamond}(#1)}

\newcommand{\maxpc}[1]{{\mathsf{top}}_{\mathsf{AP}}(#1)}
\newcommand{\maxgmod}[1]{{\mathsf{top}}_{\mathsf{gm}}(#1)}
\newcommand{\gm}[2]{\mathsf{gm}(#1,#2)}
\newcommand{\lvl}[2]{\mathsf{lvl}(#1,#2)}

\newcommand{\boxchop}[2]{\boxbin{\,\chop\,}{#1}{#2}}
\newcommand{\boxguarantee}[2]{\boxbin{\uarantee}{#1}{#2}}

\DeclareMathOperator{\ambientchop}{\mathbin{\chopop}}%{\mathbin{|}}

\newcommand{\ambientprop}{\mathtt{ap}}
\newcommand{\ambientchild}{\mathtt{rel}}
\newcommand{\numchildgeq}[1]{\mathtt{[\#\,{\geq}\,#1]}}
\newcommand{\numchildeq}[1]{\mathtt{[\#\,{=}\,#1]}}

\newcommand{\ambienttrees}{\mathbb{T}_{\mathsf{SAL}}\xspace}

\newcommand{\aname}{\mathsf{n}}
\newcommand{\anamebis}{\mathsf{m}}
\newcommand{\anameter}{\avarprop}
\newcommand{\anvarprop}{\avarprop}
\newcommand{\anvarpropbis}{\avarpropbis}

\newcommand{\ambworld}{\mathtt{world}}

\newcommand{\aCCmodeltranslation}[4]{\mathcal{T}^{#4}_{#1}\pair{#2}{#3}}
\newcommand{\aSALmodeltranslation}[2]{\mathcal{T}_{#2}(#1)}
\newcommand{\aSALmodeltranslationaux}[4]{\mathcal{T}^{#4}_{#1}\pair{#2}{#3}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  LICS - MLSTAR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\MLStar}{{\ensuremath{\ML(\separate)}}\xspace}
\newcommand{\MSLDS}{{\ensuremath{\mathsf{MSL}(\separate,\Diamond^{-1})}}\xspace}

\newcommand{\DNF}[1]{\mathsf{DNF}(#1)}

\newcommand{\previouschapter}[1]{
  \begin{tcenter}
    $\left[\,\text{%
    \scalebox{0.96}{%
    \begin{minipage}{\linewidth}%
      #1
    \end{minipage}}}%
    \,\right]%
    $
\end{tcenter}
}

\newcommand{\zero}{\mathtt{0}}
\newcommand{\one}{\mathtt{1}}

\newcommand{\Boxbox}{\boxplus}

\newcommand{\QK}{\ensuremath{\mathsf{QK}}\xspace}
\newcommand{\modallogicSC}{\MLStar}

\newcommand{\atypeset}[2]{\mathcal{T}^{#2}{(#1)}}
\newcommand{\atowertypeset}[2]{\mathscr{T}^{#2}{(#1)}}

\newcommand{\acharformula}[3]{\Gamma(#1)_{#2}^{#3}}
\newcommand{\typeeqclass}[2]{\equiv_{#1}^{#2}}
\newcommand{\towertypeeqclass}[2]{{\equiv{\!\!\uparrow}}_{#1}^{#2}}

\newcommand{\gamerel}[2]{\approx_{#1}^{#2}}
\newcommand{\neggamerel}[2]{{\not\approx}_{#1}^{#2}}

\newcommand{\abisim}{\mathcal{Z}}
\newcommand{\abisimtwo}{\mathcal{Y}}
\newcommand{\bisrel}[2]{\xspace\leftrightarrows_{#1}^{#2}\xspace}

\newcommand{\atermset}{{\mathsf{T}}}

\newcommand{\Tgarbage}{\mathcal{G}}


\newcommand{\MLSformulaerankset}[2]{\modallogicSC[#1,#2]}

\newcommand{\acharformulaSC}[3]{\Pi(#1)_{#2}^{#3}}

\newcommand{\boundd}[1]{\mathcal{B}(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  TILING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tiling}{\mathtt{Tile}}

\newcommand{\cH}{\mathsf{H}}
\newcommand{\cT}{\mathsf{T}}
\newcommand{\cTT}{\mathscr{T}}
\newcommand{\cTacc}{\mathcal{T}_{\text{acc}}}
\newcommand{\cV}{\mathsf{V}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\AP}{\varprop}
\newcommand{\tilinginit}[1]{\mathsf{init}(#1)}

\newcommand{\pZT}[2]{\texttt{\apZ}_{#2}{(#1)}}
\newcommand{\pUT}[2]{\texttt{\apU}_{#2}{(#1)}}
\newcommand{\pCTB}[3]{\texttt{\apC}[#3]_{#2}{(#1)}}
\newcommand{\pCTBB}[2]{\texttt{\apC}_{#2}{(#1)}}
\newcommand{\pTiles}[3]{\texttt{tiles}[#3]_{#2}{(#1)}}

\newcommand{\apS}{sub}
\newcommand{\apZ}{zero}
\newcommand{\apU}{uniq}
\newcommand{\apC}{compl}
\newcommand{\apA}{aux}
\newcommand{\pS}[1]{\mathtt{\apS}{(#1)}}
\newcommand{\pZ}[1]{\mathtt{\apZ}{(#1)}}
\newcommand{\pU}[1]{\mathtt{\apU}{(#1)}}
\newcommand{\pC}[1]{\mathtt{\apC}{(#1)}}
\newcommand{\pA}{\mathtt{\apA}}

\newcommand{\hset}{\mathsf{H}}
\newcommand{\vset}{\mathsf{V}}

\newcommand{\MTP}{\ensuremath{\mathsf{MTP}}\xspace}
\newcommand{\AMTP}{\ensuremath{\mathsf{AMTP}}\xspace}

\newcommand{\cM}{\mathcal{M}}

\newcommand{\bl}{\mathtt{bl}}
\newcommand{\wht}{\mathtt{wh}}

\newcommand{\atile}{\mathtt{c}}

\newcommand{\complete}[1]{\mathtt{type}(#1)}
\newcommand{\completeplus}[1]{\mathtt{type}_{\mathtt{lsr}}(#1)}

\newcommand{\treeval}{\mathtt{val}}
\newcommand{\treevalV}{\mathtt{val}_{\text{V}}}
\newcommand{\treevalH}{\mathtt{val}_{\text{H}}}

\newcommand{\Aux}{\mathtt{Aux}}
\newcommand{\Val}{\mathtt{Val}}
\newcommand{\aaux}{\mathtt{ax}}
\newcommand{\aauxbis}{\mathtt{bx}}

\newcommand{\avarleft}{\mathtt{l}}
\newcommand{\avarselect}{\mathtt{s}}
\newcommand{\avarright}{\mathtt{r}}

\newcommand{\nb}[1]{\boldsymbol{\mathfrak{n}}(#1)}
\newcommand{\nbexp}[2]{\boldsymbol{\mathfrak{n}}_{#2}(#1)}

\newcommand{\fork}[4]{\mathtt{fork}^{#3}_{#4}(#1,#2)}

\newcommand{\successor}[3]{[#2 = #1 {+} 1]_{#3}}
\newcommand{\less}[4]{[#1\,{<}\,#2]^{#3}_{#4}}
\newcommand{\equivalent}[4]{[#1\,{=}\,#2]^{#3}_{#4}}

\newcommand{\lsrpartition}[1]{\mathtt{lsr}(#1)}
\newcommand{\twonoms}[3]{\mathtt{nom}_{#3}(#1\!\neq\!#2)}

\newcommand{\ainit}{init}
\newcommand{\init}[1]{\mathtt{\ainit}(#1)}

\newcommand{\nominal}[2]{\mathtt{nom}_{#2}(#1)}

\newcommand{\bsuccessor}[4]{[#2\,{\eqtext{$#4$}}\,#1 {+} 1]_{#3}}
\newcommand{\bequivalent}[4]{[#1\,{\eqtext{$#4$}}\,#2]_{#3}}

\newcommand{\bless}[4]{[#1\,{\lesstext{$#4$}}\,#2]_{#3}}

\newcommand{\selectpred}[4]{\mathtt{S}^{#3}_{#4}(#1, #2)}
\newcommand{\bselectpred}[4]{\mathtt{S[}#4\mathtt{]}_{#3}(#1,#2)}
\newcommand{\leftpred}[4]{\mathtt{L}^{#3}_{#4}(#1, #2)}
\newcommand{\bleftpred}[4]{\mathtt{L[}#4\mathtt{]}_{#3}(#1,#2)}
\newcommand{\selectleftpred}[4]{\mathtt{LS}^{#3}_{#4}(#1, #2)}
\newcommand{\bselectleftpred}[4]{\mathtt{LS[}#4\mathtt{]}_{#3}(#1,#2)}
\newcommand{\rightpred}[2]{\mathtt{R}(#1,#2)}
\newcommand{\brightpred}[3]{\mathtt{R[}#3\mathtt{]}(#1,#2)}

\newcommand{\atiling}[2]{\mathtt{tiling}_{#2}(#1)}
\newcommand{\agrid}[2]{\mathtt{grid}_{#2}(#1)}

\newcommand{\atnom}[2]{\mathtt{@}_{#1}^{#2}}

\newcommand{\heapdim}{D}


\newcommand{\apone}{one}
\newcommand{\apfirst}{first}
\newcommand{\aphor}{hor}
\newcommand{\apvert}{vert}
\newcommand{\pone}[1]{\texttt{\apone}_{#1}}
\newcommand{\pfirst}[2]{\texttt{\apfirst}_{#2}{(#1)}}
\newcommand{\phor}[2]{\texttt{\aphor}_{#2}{(#1)}}
\newcommand{\pvert}[2]{\texttt{\apvert}_{#2}{(#1)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  TEAM LOGIC
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\plneg}{\dot{\neg}}
%\newcommand{\plneg}{\overset{\boldsymbol{\cdot}}{\neg}}
\newcommand{\plvee}{\dot{\vee}}
\newcommand{\plcnot}{{\sim}}
%\newcommand{\plvee}{\overset{\boldsymbol{\cdot}}{\vee}}
\newcommand{\ateam}{\mathfrak{T}}
\newcommand{\ateambis}{\mathfrak{S}}
\newcommand{\aplvaluation}{\mathfrak{v}}

\newcommand{\tluniq}[1]{\mathtt{unique}(#1)}
\newcommand{\tlcopies}[1]{\mathtt{copies}(#1)}

\newcommand{\PLN}{\normalfont{\textsf{PL}}(\plcnot)\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  RANDOM
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\duplicate}[1]{#1

                          #1}

